Monitoring COVID-19-induced gender differences in teleworking rates using Mobile Network Data

The COVID-19 pandemic has created a sudden need for a wider uptake of home-based telework as means of sustaining the production. Generally, teleworking arrangements impacts directly worker's efficiency and motivation. The direction of this impact, however, depends on the balance between positive effects of teleworking (e.g. increased flexibility and autonomy) and its downsides (e.g. blurring boundaries between private and work life). Moreover, these effects of teleworking can be amplified in case of vulnerable groups of workers, such as women. The first step in understanding the implications of teleworking on women is to have timely information on the extent of teleworking by age and gender. In the absence of timely official statistics, in this paper we propose a method for nowcasting the teleworking trends by age and gender for 20 Italian regions using mobile network operators (MNO) data. The method is developed and validated using MNO data together with the Italian quarterly Labour Force Survey. Our results confirm that the MNO data have the potential to be used as a tool for monitoring gender and age differences in teleworking patterns. This tool becomes even more important today as it could support the adequate gender mainstreaming in the ``Next Generation EU'' recovery plan and help to manage related social impacts of COVID-19 through policymaking.

==> teleworking and MNO/model_minimal.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Wed, Sep 15, 2021 - 2:47:41 PM
\begin{table}[!htbp] \centering 
  \caption{Regression output and descriptive statistics of the model described in equation \ref{eq:mod1}} 
  \label{minimal model} 

\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{\textit{Teleworking}} \\ 
\hline \\[-1.8ex] 
employment & \multicolumn{2}{c}{0.041$^{*}$ (0.021)} \\ 
log(mobility) & \multicolumn{2}{c}{$-$0.169$^{***}$ (0.020)}\\ 
Constant & \multicolumn{2}{c}{$-$0.091$^{***}$ (0.031)} \\ 
\cline{2-3} 
\\[-1.8ex] & Male & Female \\ 
\cline{2-3} 
Abruzzo & $-$0.011 (0.017)  & $-$0.029 (0.019) \\ 
 Basilicata & $-$0.053$^{***}$ (0.018) & $-$0.034$^{*}$ (0.020) \\ 
 Calabria & $-$0.115$^{***}$ (0.019) & $-$0.049$^{**}$ (0.022) \\ 
 Campania & $-$0.045$^{**}$ (0.018) & 0.004 (0.021) \\ 
 Emilia Romagna & $-$0.018 (0.018) & $-$0.048$^{**}$ (0.020) \\ 
 Friuli Venezia Giulia & $-$0.007 (0.017) & 0.002 (0.019) \\ 
 Lazio & 0.072$^{***}$ (0.017)  & 0.094$^{***}$ (0.018) \\ 
 Liguria & $-$0.021 (0.019) & $-$0.043$^{**}$ (0.021) \\ 
 Lombardia & 0.076$^{***}$ (0.018)  & 0.083$^{***}$ (0.018) \\ 
 Marche & $-$0.047$^{***}$ (0.017) & $-$0.044$^{**}$ (0.019) \\ 
 Molise & $-$0.033$^{*}$ (0.018) & $-$0.014 (0.019) \\ 
 Piemonte & 0.020 (0.017)  & 0.012 (0.019) \\ 
 Puglia  & $-$0.130$^{***}$ (0.021)  & $-$0.124$^{***}$ (0.026) \\ 
 Sardegna & $-$0.045$^{**}$ (0.018) & $-$0.023 (0.020) \\ 
 Sicilia & $-$0.118$^{***}$ (0.021)  & $-$0.107$^{***}$ (0.025) \\ 
 Toscana  & $-$0.015 (0.018) & $-$0.027 (0.020) \\ 
 Trentino alto Adige & 0.009 (0.017) & 0.0002 (0.018) \\ 
 Umbria & $-$0.059$^{***}$ (0.018)  & $-$0.057$^{***}$ (0.020) \\ 
 Valle d'Aosta & 0.022 (0.018) & 0.073$^{***}$ (0.018) \\ 
 Veneto & & $-$0.031$^{*}$ (0.018) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{2}{c}{320} \\ 
R$^{2}$ & \multicolumn{2}{c}{0.606} \\ 
Adjusted R$^{2}$ & \multicolumn{2}{c}{0.548} \\ 
Residual Std. Error & \multicolumn{2}{c}{0.035 (df = 278)} \\ 
F Statistic & \multicolumn{2}{c}{10.422$^{***}$ (df = 41; 278)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

\end{table} 
